Robustness of a bisimulation-type faster-than preorder

TACS is an extension of CCS where upper time bounds for delays can be specified. Luettgen and Vogler defined three variants of bismulation-type faster-than relations and showed that they all three lead to the same preorder, demonstrating the robustness of their approach. In the present paper, the operational semantics of TACS is extended; it is shown that two of the variants still give the same preorder as before, underlining robustness. An explanation is given why this result fails for the third variant. It is also shown that another variant, which mixes old and new operational semantics, can lead to smaller relations that prove the same preorder.

==> eptcsdata.tex <==
\providecommand{\event}{S.~Fr\"oschle, D.~Gorla (Eds.): Workshop on Expressiveness\\
in Concurrency 2009 (EXPRESS'09).}
\providecommand{\volume}{8}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{66}
\providecommand{\eid}{6}

